Two-stage coding over the Z-channel

In this paper, we discuss two-stage encoding algorithms capable of correcting a fraction of asymmetric errors. Suppose that the encoder transmits $n$ binary symbols $(x_1,\ldots,x_n)$ one-by-one over the Z-channel, in which a 1 is received only if a 1 is transmitted. At some designated moment, say $n_1$, the encoder uses noiseless feedback and adjusts further encoding strategy based on the partial output of the channel $(y_1,\ldots,y_{n_1})$. The goal is to transmit error-free as much information as possible under the assumption that the total number of errors inflicted by the Z-channel is limited by $\tau n$, $0<\tau<1$. We propose an encoding strategy that uses a list-decodable code at the first stage and a high-error low-rate code at the second stage. This strategy and our converse result yield that there is a sharp transition at $\tau=\max\limits_{0<w<1}\frac{w + w^3}{1+4w^3}\approx 0.44$ from positive rate to zero rate for two-stage encoding strategies. As side results, we derive bounds on the size of list-decodable codes for the Z-channel and prove that for a fraction $1/4+\epsilon$ of asymmetric errors, an error-correcting code contains at most $O(\epsilon^{-3/2})$ codewords.

==> low_feedback.tex <==
0.001000 0.989591
0.002000 0.981180
0.003000 0.973523
0.004000 0.966355
0.005000 0.959549
0.006000 0.953033
0.007000 0.946757
0.008000 0.940686
0.009000 0.934795
0.010000 0.929063
0.011000 0.923474
0.012000 0.918014
0.013000 0.912674
0.014000 0.907444
0.015000 0.902315
0.016000 0.897281
0.017000 0.892335
0.018000 0.887474
0.019000 0.882691
0.020000 0.877982
0.021000 0.873345
0.022000 0.868774
0.023000 0.864268
0.024000 0.859823
0.025000 0.855437
0.026000 0.851108
0.027000 0.846832
0.028000 0.842608
0.029000 0.838435
0.030000 0.834310
0.031000 0.830231
0.032000 0.826198
0.033000 0.822208
0.034000 0.818261
0.035000 0.814355
0.036000 0.810488
0.037000 0.806660
0.038000 0.802870
0.039000 0.799117
0.040000 0.795399
0.041000 0.791716
0.042000 0.788066
0.043000 0.784450
0.044000 0.780865
0.045000 0.777313
0.046000 0.773790
0.047000 0.770298
0.048000 0.766835
0.049000 0.763401
0.050000 0.759995
0.051000 0.756616
0.052000 0.753264
0.053000 0.749939
0.054000 0.746639
0.055000 0.743365
0.056000 0.740116
0.057000 0.736891
0.058000 0.733690
0.059000 0.730513
0.060000 0.727358
0.061000 0.724227
0.062000 0.721117
0.063000 0.718030
0.064000 0.714964
0.065000 0.711919
0.066000 0.708895
0.067000 0.705892
0.068000 0.702909
0.069000 0.699945
0.070000 0.697001
0.071000 0.694077
0.072000 0.691171
0.073000 0.688284
0.074000 0.685416
0.075000 0.682566
0.076000 0.679733
0.077000 0.676919
0.078000 0.674121
0.079000 0.671341
0.080000 0.668578
0.081000 0.665831
0.082000 0.663101
0.083000 0.660387
0.084000 0.657689
0.085000 0.655007
0.086000 0.652341
0.087000 0.649690
0.088000 0.647055
0.089000 0.644434
0.090000 0.641829
0.091000 0.639238
0.092000 0.636661
0.093000 0.634099
0.094000 0.631551
0.095000 0.629017
0.096000 0.626498
0.097000 0.623991
0.098000 0.621499
0.099000 0.619019
0.100000 0.616553
0.101000 0.614100
0.102000 0.611660
0.103000 0.609233
0.104000 0.606819
0.105000 0.604417
0.106000 0.602028
0.107000 0.599651
0.108000 0.597286
0.109000 0.594933
0.110000 0.592592
0.111000 0.590263
0.112000 0.587946
0.113000 0.585640
0.114000 0.583345
0.115000 0.581062
0.116000 0.578791
0.117000 0.576530
0.118000 0.574281
0.119000 0.572042
0.120000 0.569814
0.121000 0.567597
0.122000 0.565391
0.123000 0.563195
0.124000 0.561009
0.125000 0.558834
0.126000 0.556670
0.127000 0.554515
0.128000 0.552370
0.129000 0.550236
0.130000 0.548111
0.131000 0.545996
0.132000 0.543891
0.133000 0.541796
0.134000 0.539710
0.135000 0.537633
0.136000 0.535567
0.137000 0.533509
0.138000 0.531461
0.139000 0.529421
0.140000 0.527391
0.141000 0.525370
0.142000 0.523358
0.143000 0.521355
0.144000 0.519361
0.145000 0.517375
0.146000 0.515398
0.147000 0.513430
0.148000 0.511470
0.149000 0.509519
0.150000 0.507576
0.151000 0.505642
0.152000 0.503716
0.153000 0.501798
0.154000 0.499888
0.155000 0.497986
0.156000 0.496093
0.157000 0.494207
0.158000 0.492330
0.159000 0.490460
0.160000 0.488598
0.161000 0.486744
0.162000 0.484898
0.163000 0.483059
0.164000 0.481228
0.165000 0.479404
0.166000 0.477588
0.167000 0.475780
0.168000 0.473979
0.169000 0.472185
0.170000 0.470398
0.171000 0.468619
0.172000 0.466847
0.173000 0.465082
0.174000 0.463324
0.175000 0.461573
0.176000 0.459830
0.177000 0.458093
0.178000 0.456363
0.179000 0.454640
0.180000 0.452924
0.181000 0.451215
0.182000 0.449512
0.183000 0.447816
0.184000 0.446127
0.185000 0.444444
0.186000 0.442768
0.187000 0.441099
0.188000 0.439436
0.189000 0.437779
0.190000 0.436129
0.191000 0.434486
0.192000 0.432848
0.193000 0.431217
0.194000 0.429592
0.195000 0.427974
0.196000 0.426361
0.197000 0.424755
0.198000 0.423155
0.199000 0.421561
0.200000 0.419973
0.201000 0.418391
0.202000 0.416815
0.203000 0.415245
0.204000 0.413681
0.205000 0.412123
0.206000 0.410570
0.207000 0.409024
0.208000 0.407483
0.209000 0.405948
0.210000 0.404418
0.211000 0.402895
0.212000 0.401377
0.213000 0.399864
0.214000 0.398357
0.215000 0.396856
0.216000 0.395360
0.217000 0.393870
0.218000 0.392385
0.219000 0.390906
0.220000 0.389432
0.221000 0.387963
0.222000 0.386500
0.223000 0.385042
0.224000 0.383589
0.225000 0.382142
0.226000 0.380699
0.227000 0.379263
0.228000 0.377831
0.229000 0.376404
0.230000 0.374983
0.231000 0.373566
0.232000 0.372155
0.233000 0.370749
0.234000 0.369347
0.235000 0.367951
0.236000 0.366560
0.237000 0.365173
0.238000 0.363792
0.239000 0.362415
0.240000 0.361044
0.241000 0.359677
0.242000 0.358315
0.243000 0.356958
0.244000 0.355605
0.245000 0.354258
0.246000 0.352915
0.247000 0.351577
0.248000 0.350243
0.249000 0.348914
0.250000 0.347590
0.251000 0.346270
0.252000 0.344955
0.253000 0.343645
0.254000 0.342339
0.255000 0.341037
0.256000 0.339741
0.257000 0.338448
0.258000 0.337160
0.259000 0.335877
0.260000 0.334598
0.261000 0.333323
0.262000 0.332053
0.263000 0.330787
0.264000 0.329525
0.265000 0.328268
0.266000 0.327015
0.267000 0.325767
0.268000 0.324522
0.269000 0.323282
0.270000 0.322046
0.271000 0.320815
0.272000 0.319587
0.273000 0.318364
0.274000 0.317145
0.275000 0.315929
0.276000 0.314719
0.277000 0.313512
0.278000 0.312309
0.279000 0.311110
0.280000 0.309916
0.281000 0.308725
0.282000 0.307538
0.283000 0.306356
0.284000 0.305177
0.285000 0.304002
0.286000 0.302832
0.287000 0.301665
0.288000 0.300502
0.289000 0.299343
0.290000 0.298188
0.291000 0.297036
0.292000 0.295889
0.293000 0.294745
0.294000 0.293605
0.295000 0.292469
0.296000 0.291337
0.297000 0.290208
0.298000 0.289084
0.299000 0.287963
0.300000 0.286845
0.301000 0.285732
0.302000 0.284622
0.303000 0.283515
0.304000 0.282413
0.305000 0.281314
0.306000 0.280218
0.307000 0.279127
0.308000 0.278038
0.309000 0.276954
0.310000 0.275873
0.311000 0.274795
0.312000 0.273722
0.313000 0.272651
0.314000 0.271584
0.315000 0.270521
0.316000 0.269461
0.317000 0.268405
0.318000 0.267352
0.319000 0.266302
0.320000 0.265256
0.321000 0.264213
0.322000 0.263174
0.323000 0.262138
0.324000 0.261106
0.325000 0.260076
0.326000 0.259051
0.327000 0.258028
0.328000 0.257009
0.329000 0.255993
0.330000 0.254981
0.331000 0.253971
0.332000 0.252965
0.333000 0.251963
0.334000 0.250963
0.335000 0.249967
0.336000 0.248974
0.337000 0.247984
0.338000 0.246998
0.339000 0.246014
0.340000 0.245034
0.341000 0.244057
0.342000 0.243083
0.343000 0.242112
0.344000 0.241145
0.345000 0.240180
0.346000 0.239219
0.347000 0.238261
0.348000 0.237305
0.349000 0.236353
0.350000 0.235404
0.351000 0.234458
0.352000 0.233515
0.353000 0.232575
0.354000 0.231638
0.355000 0.230704
0.356000 0.229774
0.357000 0.228846
0.358000 0.227921
0.359000 0.226999
0.360000 0.226080
0.361000 0.225164
0.362000 0.224251
0.363000 0.223340
0.364000 0.222433
0.365000 0.221529
0.366000 0.220627
0.367000 0.219729
0.368000 0.218833
0.369000 0.217940
0.370000 0.217050
0.371000 0.216163
0.372000 0.215279
0.373000 0.214397
0.374000 0.213518
0.375000 0.212642
0.376000 0.211769
0.377000 0.210899
0.378000 0.210032
0.379000 0.209167
0.380000 0.208305
0.381000 0.207446
0.382000 0.206589
0.383000 0.205735
0.384000 0.204884
0.385000 0.204036
0.386000 0.203191
0.387000 0.202348
0.388000 0.201507
0.389000 0.200670
0.390000 0.199835
0.391000 0.199003
0.392000 0.198173
0.393000 0.197346
0.394000 0.196522
0.395000 0.195700
0.396000 0.194881
0.397000 0.194065
0.398000 0.193251
0.399000 0.192440
0.400000 0.191631
0.401000 0.190825
0.402000 0.190022
0.403000 0.189221
0.404000 0.188422
0.405000 0.187626
0.406000 0.186833
0.407000 0.186042
0.408000 0.185254
0.409000 0.184468
0.410000 0.183685
0.411000 0.182904
0.412000 0.182126
0.413000 0.181350
0.414000 0.180577
0.415000 0.179806
0.416000 0.179038
0.417000 0.178272
0.418000 0.177508
0.419000 0.176747
0.420000 0.175989
0.421000 0.175232
0.422000 0.174479
0.423000 0.173727
0.424000 0.172978
0.425000 0.172232
0.426000 0.171487
0.427000 0.170745
0.428000 0.170006
0.429000 0.169269
0.430000 0.168534
0.431000 0.167802
0.432000 0.167071
0.433000 0.166344
0.434000 0.165618
0.435000 0.164895
0.436000 0.164174
0.437000 0.163456
0.438000 0.162740
0.439000 0.162026
0.440000 0.161314
0.441000 0.160605
0.442000 0.159898
0.443000 0.159193
0.444000 0.158490
0.445000 0.157790
0.446000 0.157092
0.447000 0.156396
0.448000 0.155702
0.449000 0.155011
0.450000 0.154322
0.451000 0.153635
0.452000 0.152950
0.453000 0.152268
0.454000 0.151587
0.455000 0.150909
0.456000 0.150233
0.457000 0.149559
0.458000 0.148888
0.459000 0.148218
0.460000 0.147551
0.461000 0.146886
0.462000 0.146223
0.463000 0.145562
0.464000 0.144903
0.465000 0.144246
0.466000 0.143592
0.467000 0.142939
0.468000 0.142289
0.469000 0.141641
0.470000 0.140995
0.471000 0.140351
0.472000 0.139709
0.473000 0.139069
0.474000 0.138431
0.475000 0.137795
0.476000 0.137161
0.477000 0.136530
0.478000 0.135900
0.479000 0.135273
0.480000 0.134647
0.481000 0.134024
0.482000 0.133402
0.483000 0.132783
0.484000 0.132165
0.485000 0.131550
0.486000 0.130937
0.487000 0.130325
0.488000 0.129716
0.489000 0.129108
0.490000 0.128503
0.491000 0.127899
0.492000 0.127298
0.493000 0.126698
0.494000 0.126101
0.495000 0.125505
0.496000 0.124912
0.497000 0.124320
0.498000 0.123730
0.499000 0.123142
0.500000 0.122556
0.501000 0.121972
0.502000 0.121390
0.503000 0.120810
0.504000 0.120232
0.505000 0.119655
0.506000 0.119081
0.507000 0.118508
0.508000 0.117938
0.509000 0.117369
0.510000 0.116802
0.511000 0.116237
0.512000 0.115674
0.513000 0.115112
0.514000 0.114553
0.515000 0.113995
0.516000 0.113440
0.517000 0.112886
0.518000 0.112334
0.519000 0.111783
0.520000 0.111235
0.521000 0.110688
0.522000 0.110144
0.523000 0.109601
0.524000 0.109060
0.525000 0.108520
0.526000 0.107983
0.527000 0.107447
0.528000 0.106913
0.529000 0.106381
0.530000 0.105851
0.531000 0.105322
0.532000 0.104795
0.533000 0.104270
0.534000 0.103747
0.535000 0.103225
0.536000 0.102706
0.537000 0.102188
0.538000 0.101671
0.539000 0.101157
0.540000 0.100644
0.541000 0.100133
0.542000 0.099624
0.543000 0.099116
0.544000 0.098610
0.545000 0.098106
0.546000 0.097604
0.547000 0.097103
0.548000 0.096604
0.549000 0.096107
0.550000 0.095611
0.551000 0.095117
0.552000 0.094625
0.553000 0.094135
0.554000 0.093646
0.555000 0.093158
0.556000 0.092673
0.557000 0.092189
0.558000 0.091707
0.559000 0.091226
0.560000 0.090747
0.561000 0.090270
0.562000 0.089795
0.563000 0.089321
0.564000 0.088848
0.565000 0.088378
0.566000 0.087909
0.567000 0.087441
0.568000 0.086976
0.569000 0.086511
0.570000 0.086049
0.571000 0.085588
0.572000 0.085129
0.573000 0.084671
0.574000 0.084215
0.575000 0.083760
0.576000 0.083307
0.577000 0.082856
0.578000 0.082406
0.579000 0.081958
0.580000 0.081512
0.581000 0.081067
0.582000 0.080623
0.583000 0.080181
0.584000 0.079741
0.585000 0.079302
0.586000 0.078865
0.587000 0.078429
0.588000 0.077995
0.589000 0.077563
0.590000 0.077132
0.591000 0.076702
0.592000 0.076274
0.593000 0.075848
0.594000 0.075423
0.595000 0.075000
0.596000 0.074578
0.597000 0.074157
0.598000 0.073739
0.599000 0.073321
0.600000 0.072906
0.601000 0.072491
0.602000 0.072079
0.603000 0.071667
0.604000 0.071257
0.605000 0.070849
0.606000 0.070442
0.607000 0.070037
0.608000 0.069633
0.609000 0.069231
0.610000 0.068830
0.611000 0.068430
0.612000 0.068032
0.613000 0.067636
0.614000 0.067241
0.615000 0.066847
0.616000 0.066455
0.617000 0.066064
0.618000 0.065675
0.619000 0.065287
0.620000 0.064901
0.621000 0.064516
0.622000 0.064132
0.623000 0.063750
0.624000 0.063370
0.625000 0.062991
0.626000 0.062613
0.627000 0.062236
0.628000 0.061861
0.629000 0.061488
0.630000 0.061116
0.631000 0.060745
0.632000 0.060376
0.633000 0.060008
0.634000 0.059641
0.635000 0.059276
0.636000 0.058912
0.637000 0.058550
0.638000 0.058189
0.639000 0.057829
0.640000 0.057471
0.641000 0.057114
0.642000 0.056759
0.643000 0.056404
0.644000 0.056052
0.645000 0.055700
0.646000 0.055350
0.647000 0.055002
0.648000 0.054654
0.649000 0.054308
0.650000 0.053964
0.651000 0.053620
0.652000 0.053278
0.653000 0.052938
0.654000 0.052599
0.655000 0.052261
0.656000 0.051924
0.657000 0.051589
0.658000 0.051255
0.659000 0.050922
0.660000 0.050591
0.661000 0.050261
0.662000 0.049932
0.663000 0.049605
0.664000 0.049279
0.665000 0.048954
0.666000 0.048631
0.667000 0.048308
0.668000 0.047988
0.669000 0.047668
0.670000 0.047350
0.671000 0.047033
0.672000 0.046717
0.673000 0.046403
0.674000 0.046090
0.675000 0.045778
0.676000 0.045467
0.677000 0.045158
0.678000 0.044850
0.679000 0.044543
0.680000 0.044238
0.681000 0.043933
0.682000 0.043630
0.683000 0.043329
0.684000 0.043028
0.685000 0.042729
0.686000 0.042431
0.687000 0.042134
0.688000 0.041839
0.689000 0.041545
0.690000 0.041252
0.691000 0.040960
0.692000 0.040670
0.693000 0.040380
0.694000 0.040092
0.695000 0.039805
0.696000 0.039520
0.697000 0.039236
0.698000 0.038952
0.699000 0.038670
0.700000 0.038390
0.701000 0.038110
0.702000 0.037832
0.703000 0.037555
0.704000 0.037279
0.705000 0.037004
0.706000 0.036731
0.707000 0.036459
0.708000 0.036187
0.709000 0.035918
0.710000 0.035649
0.711000 0.035381
0.712000 0.035115
0.713000 0.034850
0.714000 0.034586
0.715000 0.034323
0.716000 0.034062
0.717000 0.033801
0.718000 0.033542
0.719000 0.033284
0.720000 0.033027
0.721000 0.032771
0.722000 0.032516
0.723000 0.032263
0.724000 0.032011
0.725000 0.031760
0.726000 0.031510
0.727000 0.031261
0.728000 0.031013
0.729000 0.030767
0.730000 0.030521
0.731000 0.030277
0.732000 0.030034
0.733000 0.029792
0.734000 0.029551
0.735000 0.029311
0.736000 0.029073
0.737000 0.028836
0.738000 0.028599
0.739000 0.028364
0.740000 0.028130
0.741000 0.027897
0.742000 0.027665
0.743000 0.027435
0.744000 0.027205
0.745000 0.026977
0.746000 0.026749
0.747000 0.026523
0.748000 0.026298
0.749000 0.026074
0.750000 0.025851
0.751000 0.025629
0.752000 0.025408
0.753000 0.025189
0.754000 0.024970
0.755000 0.024752
0.756000 0.024536
0.757000 0.024321
0.758000 0.024107
0.759000 0.023893
0.760000 0.023681
0.761000 0.023470
0.762000 0.023261
0.763000 0.023052
0.764000 0.022844
0.765000 0.022637
0.766000 0.022432
0.767000 0.022227
0.768000 0.022024
0.769000 0.021821
0.770000 0.021620
0.771000 0.021420
0.772000 0.021220
0.773000 0.021022
0.774000 0.020825
0.775000 0.020629
0.776000 0.020434
0.777000 0.020240
0.778000 0.020047
0.779000 0.019855
0.780000 0.019664
0.781000 0.019475
0.782000 0.019286
0.783000 0.019098
0.784000 0.018911
0.785000 0.018726
0.786000 0.018541
0.787000 0.018357
0.788000 0.018175
0.789000 0.017993
0.790000 0.017813
0.791000 0.017633
0.792000 0.017455
0.793000 0.017277
0.794000 0.017101
0.795000 0.016925
0.796000 0.016751
0.797000 0.016577
0.798000 0.016405
0.799000 0.016234
0.800000 0.016063
0.801000 0.015894
0.802000 0.015725
0.803000 0.015558
0.804000 0.015391
0.805000 0.015226
0.806000 0.015062
0.807000 0.014898
0.808000 0.014736
0.809000 0.014574
0.810000 0.014414
0.811000 0.014254
0.812000 0.014096
0.813000 0.013938
0.814000 0.013782
0.815000 0.013626
0.816000 0.013471
0.817000 0.013318
0.818000 0.013165
0.819000 0.013013
0.820000 0.012863
0.821000 0.012713
0.822000 0.012564
0.823000 0.012416
0.824000 0.012269
0.825000 0.012123
0.826000 0.011978
0.827000 0.011834
0.828000 0.011691
0.829000 0.011549
0.830000 0.011408
0.831000 0.011268
0.832000 0.011129
0.833000 0.010990
0.834000 0.010853
0.835000 0.010717
0.836000 0.010581
0.837000 0.010447
0.838000 0.010313
0.839000 0.010181
0.840000 0.010049
0.841000 0.009918
0.842000 0.009788
0.843000 0.009659
0.844000 0.009531
0.845000 0.009404
0.846000 0.009278
0.847000 0.009153
0.848000 0.009029
0.849000 0.008905
0.850000 0.008783
0.851000 0.008661
0.852000 0.008541
0.853000 0.008421
0.854000 0.008302
0.855000 0.008184
0.856000 0.008067
0.857000 0.007951
0.858000 0.007836
0.859000 0.007722
0.860000 0.007608
0.861000 0.007496
0.862000 0.007385
0.863000 0.007274
0.864000 0.007164
0.865000 0.007055
0.866000 0.006947
0.867000 0.006840
0.868000 0.006734
0.869000 0.006629
0.870000 0.006524
0.871000 0.006421
0.872000 0.006318
0.873000 0.006217
0.874000 0.006116
0.875000 0.006016
0.876000 0.005917
0.877000 0.005818
0.878000 0.005721
0.879000 0.005625
0.880000 0.005529
0.881000 0.005434
0.882000 0.005340
0.883000 0.005247
0.884000 0.005155
0.885000 0.005064
0.886000 0.004974
0.887000 0.004884
0.888000 0.004795
0.889000 0.004708
0.890000 0.004621
0.891000 0.004535
0.892000 0.004449
0.893000 0.004365
0.894000 0.004282
0.895000 0.004199
0.896000 0.004117
0.897000 0.004036
0.898000 0.003956
0.899000 0.003877
0.900000 0.003798
0.901000 0.003721
0.902000 0.003644
0.903000 0.003568
0.904000 0.003493
0.905000 0.003419
0.906000 0.003345
0.907000 0.003273
0.908000 0.003201
0.909000 0.003130
0.910000 0.003060
0.911000 0.002991
0.912000 0.002923
0.913000 0.002855
0.914000 0.002788
0.915000 0.002722
0.916000 0.002657
0.917000 0.002593
0.918000 0.002530
0.919000 0.002467
0.920000 0.002405
0.921000 0.002344
0.922000 0.002284
0.923000 0.002225
0.924000 0.002166
0.925000 0.002108
0.926000 0.002051
0.927000 0.001995
0.928000 0.001940
0.929000 0.001886
0.930000 0.001832
0.931000 0.001779
0.932000 0.001727
0.933000 0.001676
0.934000 0.001625
0.935000 0.001575
0.936000 0.001526
0.937000 0.001478
0.938000 0.001431
0.939000 0.001385
0.940000 0.001339
0.941000 0.001294
0.942000 0.001250
0.943000 0.001206
0.944000 0.001164
0.945000 0.001122
0.946000 0.001081
0.947000 0.001041
0.948000 0.001001
0.949000 0.000963
0.950000 0.000925
0.951000 0.000888
0.952000 0.000852
0.953000 0.000816
0.954000 0.000781
0.955000 0.000747
0.956000 0.000714
0.957000 0.000682
0.958000 0.000650
0.959000 0.000619
0.960000 0.000589
0.961000 0.000560
0.962000 0.000531
0.963000 0.000503
0.964000 0.000476
0.965000 0.000450
0.966000 0.000424
0.967000 0.000399
0.968000 0.000375
0.969000 0.000352
0.970000 0.000330
0.971000 0.000308
0.972000 0.000287
0.973000 0.000267
0.974000 0.000247
0.975000 0.000228
0.976000 0.000210
0.977000 0.000193
0.978000 0.000177
0.979000 0.000161
0.980000 0.000146
0.981000 0.000131
0.982000 0.000118
0.983000 0.000105
0.984000 0.000093
0.985000 0.000082
0.986000 0.000071
0.987000 0.000061
0.988000 0.000052
0.989000 0.000044
0.990000 0.000036
0.991000 0.000029
0.992000 0.000023
0.993000 0.000018
0.994000 0.000013
0.995000 0.000009
0.996000 0.000006
0.997000 0.000003
0.998000 0.000001

